ReachNN: Reachability Analysis of Neural-Network Controlled Systems

Applying neural networks as controllers in dynamical systems has shown great promises. However, it is critical yet challenging to verify the safety of such control systems with neural-network controllers in the loop. Previous methods for verifying neural network controlled systems are limited to a few specific activation functions. In this work, we propose a new reachability analysis approach based on Bernstein polynomials that can verify neural-network controlled systems with a more general form of activation functions, i.e., as long as they ensure that the neural networks are Lipschitz continuous. Specifically, we consider abstracting feedforward neural networks with Bernstein polynomials for a small subset of inputs. To quantify the error introduced by abstraction, we provide both theoretical error bound estimation based on the theory of Bernstein polynomials and more practical sampling based error bound estimation, following a tight Lipschitz constant estimation approach based on forward reachability analysis. Compared with previous methods, our approach addresses a much broader set of neural networks, including heterogeneous neural networks that contain multiple types of activation functions. Experiment results on a variety of benchmarks show the effectiveness of our approach.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
		Corrected the bug with acmPrice.
		Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
		The package now is compatible with polyglossia (Joachim Breitner).
		Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
		Deleted indent for subsubsection (suggested by Ross Moore)
		Suppressed some obscurious warning in BibTeX processing
		Suppressed hyperrerf warnings (Paolo G. Giarrusso)
		New code for sections to help with accessibility patches
		(Ross Moore)
		Submission id, if present, is printed in anon mode
		Bug fixes

Version 1.55    Bug fixes


==> sections/motivating.tex <==


\begin{figure}[tbp]
	\centering	
	\subfloat[path tracking model]{%
		\includegraphics[width=0.2\textwidth]{figs/errorPosture.pdf}%
		\label{fig:error_dynamic}%
	}\quad
	\subfloat[feedback control structure]{%
		\includegraphics[width=0.2\textwidth]{figs/structure.pdf}%
		\label{fig:control_structure}%
	}
	\caption{Path tracking and neural network feedback control}
	\label{fig:case_study}
\end{figure}

\noindent
\textbf{[Motivating Example: Path Tracking for Dubins Car]} We apply our method to a case study of verifying the neural network based path tracking for a Dubins car (Figure~\ref{fig:case_study}). 
%The system under our consideration is a Dubins car controlled by a neural network. 
The continuous dynamics of a Dubins car is defined by
\begin{equation}\label{eq:dynamic}
    \begin{pmatrix}
		\dot{x} \\
		\dot{y} \\
		\dot{\theta}
    \end{pmatrix}
    =
    \begin{pmatrix}
		v \cos \theta \\
		v \sin \theta \\
		u
    \end{pmatrix},
\end{equation}
where $(x, y)$ is the coordinate of the car and denotes the car's position in a 2D plane. The variable $\theta$ is the angle between the car's heading orientation and the $x$-axis. The velocity of the car is denoted by a constant $v$, and angular velocity $\dot{\theta}$ is determined by the control input $u$. The overall control goal is to keep the car moving along a reference path that is composed of finite line segments.

The neural network controller uses two variables to measure the distance from the control goal: $d_{\text{err}}$ for the distance from the car to the reference path, and $\theta_{r}$ for the heading orientation of the current reference path segment. It works in the following way. Every $\Delta$ time, the controller obtains the values of $x$, $y$, evaluates
$d_{\text{err}} = -x \sin{\theta_r} + y \cos{\theta_r}$, $\theta_{\text{err}} = \theta_r-\theta$.
Then, it computes the control input $u$ based on $d_{\text{err}}$, $\theta_{\text{err}}$, and feeds it back to the dynamics in (\ref{eq:dynamic}).

Our goal is to prove the correctness of the controlled system's behavior with dynamics given in  Equation~\eqref{eq:dynamic}. As the first step, we approximate the behavior of the networked controlled system by our Bernstein polynomial based approximation.

%That is, we want to prove that the distance between the car and the reference path is always below a threshold, $0.5$, over the bounded time horizon $20$, i.e., $|d_{\text{err}} (t)| < 0.5$ for $t \in [0,20]$.

\begin{figure}[tbp]
	\centering	
	\includegraphics[width=0.5\textwidth]{figs/exp_result.pdf}%
	\caption{Approximated reachable states (green) and visited states (red)}
	\label{fig:exp_result}
\end{figure}

In Figure~\ref{fig:exp_result}, we show the approximated reachable states in green along with the visited states by neural network controller in red. The inputs are deliberately picked outside the range of the states that neural network was trained on. Even so, the polynomial approximation is still able to provide a good estimation of the close loop neural network controlled system and predict potential reachable set consistent with the actual visited states. To guarantee safety of neural network controllers, we can utilize the result of approximated reachable set to detect possible safety violations.

%We consider a scenario where a Dubins car needs to track a given linear reference path with a fixed speed by changing the steering velocity. The dynamic models of the car and the reference are represented as following differential equations:

%where $[\dot{x},\dot{y},\dot{\theta}]$ is the state of the car. $v$ is the linear velocity. We assume $v=V$ is fixed. $u$ is the steering velocity of the car, acting as a control input. Assume that the linear reference path starts at the origin $(0,0)$ with an angle $\theta_r$. Specially, we consider the dynamic model of tracking error (Figure \ref{fig:error_dynamic}). First we rotate the coordinate system by $\theta_r$ in a counter-clockwise direction. In the rotated coordinate system, the reference path becomes the $x$-axis, and the rotated $y$ coordinate of the vehicle is taken as the distance error, that is

%Let $\theta_{\text{err}} = \theta_r-\theta$. We can derive the following dynamic system:
%\begin{equation}\label{eq:exampleLinearTrack}
%   \begin{pmatrix}
%		\dot{d}_\text{err} \\
%		\dot{\theta}_\text{err} 
%    \end{pmatrix}
%    =
%    \begin{pmatrix}
%		 -V \sin{(\theta_r {-} \theta_\text{err})} \sin{\theta_r} + V \cos{(\theta_r {-} \theta_\text{err})} \cos{\theta_r} \\
%		-u 
%    \end{pmatrix},
%\end{equation}
%or in a compact form:
%\begin{displaymath}
%    \begin{pmatrix}
%		\dot{d}_\text{err} \\
%		\dot{\theta}_\text{err} 
%    \end{pmatrix}
%    =
%    f\left(
%    \begin{pmatrix}
%		{d}_\text{err} \\
%		{\theta}_\text{err} 
%    \end{pmatrix},u\right).
%\end{displaymath}
%In this scenario, $u=\kappa(d_\text{err},\theta_\text{err})$ is determined by a \emph{neural network} feedback controller $\kappa$ (Figure \ref{fig:control_structure}). $\kappa$ is a feed-forward network with single hidden layer consisting of $10$ neurons. The hidden layer and output layer use Hyperbolic tangent as activation function, and the output will be re-scaled to $[0, 2\pi]$ as steering angle. The approximated Lipschitz constant of this neural network is $2.01$.

%Without loss of generality, we assume that reference path starts at the coordinate $(0,0)$.
%We want to verify that for any $\theta_r \in [-\pi,\pi]$, the neural network controller can guarantee $|d_{err}|\leq 0.5$ while tracking the reference path.

